On dual Schur domain decomposition method for linear first-order transient problems

This paper addresses some numerical and theoretical aspects of dual Schur domain decomposition methods for linear first-order transient partial differential equations. In this work, we consider the trapezoidal family of schemes for integrating the ordinary differential equations (ODEs) for each subdomain and present four different coupling methods, corresponding to different algebraic constraints, for enforcing kinematic continuity on the interface between the subdomains. Method 1 (d-continuity) is based on the conventional approach using continuity of the primary variable and we show that this method is unstable for a lot of commonly used time integrators including the mid-point rule. To alleviate this difficulty, we propose a new Method 2 (Modified d-continuity) and prove its stability for coupling all time integrators in the trapezoidal family (except the forward Euler). Method 3 (v-continuity) is based on enforcing the continuity of the time derivative of the primary variable. However, this constraint introduces a drift in the primary variable on the interface. We present Method 4 (Baumgarte stabilized) which uses Baumgarte stabilization to limit this drift and we derive bounds for the stabilization parameter to ensure stability. Our stability analysis is based on the ``energy'' method, and one of the main contributions of this paper is the extension of the energy method (which was previously introduced in the context of numerical methods for ODEs) to assess the stability of numerical formulations for index-2 differential-algebraic equations (DAEs).

==> Sections/S5_DD_Stability_Analysis_July_13_2008.tex <==
%*******************************;
%  Section: Stability analysis  ;
%*******************************;
\section{STABILITY ANALYSIS}
\label{Sec:DD_S4_Stability_Analysis}
In this section we assess the stability of the $\boldsymbol{d}$-continuity, modified 
$\boldsymbol{d}$-continuity, $\boldsymbol{v}$-continuity and Baumgarte stabilized 
domain decomposition methods using the ``energy'' method \cite{Richtmyer_Morton,Hughes}. Note that 
the energy method provides sufficient conditions for stability. However, in many 
instances the obtained bounds are quite sharp. For example, in the case of ODEs, 
the obtained stability condition using the energy method (that is, the critical 
time step) has turned out to be both necessary and sufficient \cite{Hughes}. 

Let $\mathbb{R}^m$ denote the standard $m$-dimensional Euclidean space. We say the 
vectors $\boldsymbol{x}^{(n)} \in \mathbb{R}^{m} \; (n = 0, 1, 2, \cdots)$ are bounded 
$\forall n$ if there exists a positive constant $C$ independent of $n$ such that 
%------------------------------------;
%  Equation: Boundedness of vectors  ;
%------------------------------------;
\begin{align}
  \| \boldsymbol{v}^{(n)}\| < C \quad \forall n
\end{align}
%
where $\| \cdot \|$ is some convenient norm defined on $\mathbb{R}^m$ (for example, 
say the $2$-norm). Note that in finite dimensional vector spaces all norms are 
equivalent \cite{Halmos}. 

We employ the following notation for the jump and average operators over a time step:  
%----------------------------------------;
%  Equation: Jump and average operators  ;
%----------------------------------------;
\begin{align}
  \left[\boldsymbol{x}^{(n)}\right] = \boldsymbol{x}^{(n+1)} - \boldsymbol{x}^{(n)}, \quad   
  \left\{\boldsymbol{x}^{(n)}\right\} = \frac{1}{2} \left(\boldsymbol{x}^{(n+1)} + \boldsymbol{x}^{(n)} \right)
\end{align}
%
It is easy to show the following identities: 
%---------------------;
%  Equation: x_gamma  ;
%---------------------;
\begin{align}
  \label{Eqn:Trapezoidal_x_gamma}
  (1 - \gamma) \boldsymbol{x}^{(n)} + \gamma \boldsymbol{x}^{(n+1)} 
  = \left(\gamma - \frac{1}{2}\right) \left[\boldsymbol{x}^{(n)}\right] + \left\{\boldsymbol{x}^{(n)}\right\}
\end{align}
%
and for any symmetric matrix $\boldsymbol{S}$ we have 
%-------------------------;
%  Equation: Symmetric S  ;
%-------------------------;
\begin{align}
  \label{Eqn:Trapezoidal_Symmetric_S}
  \left\{\boldsymbol{x}^{(n)}\right\}^{\mathrm{T}} \boldsymbol{S} 
  \left[\boldsymbol{x}^{(n)}\right] = 
  % 
  \frac{1}{2} \left[{\boldsymbol{x}^{(n)}}^{\mathrm{T}} \boldsymbol{S} \boldsymbol{x}^{(n)} \right] 
\end{align}

For convenience we define the matrix $\boldsymbol{A}_i$ as 
%-------------------------------;
%  Equation: Definition of A_i  ;
%-------------------------------;
\begin{align}
  \label{Eqn:Trapezoidal_A_i}
  \boldsymbol{A}_i := \boldsymbol{M}_i + \left(\gamma - \frac{1}{2}\right) \Delta t \boldsymbol{K}_i
\end{align}

We choose the time step $\Delta t$ in such a way that it satisfies the stability requirements 
for all individual unconstrained subdomains (i.e., $\boldsymbol{\lambda} = \boldsymbol{0}$). 
%
That is,
%---------------------;
%  Equation: Delta t  ;
%---------------------;
\begin{align}
  \Delta t < \mathrm{min} \left(\Delta t_{1}^{\mathrm{crit}}, \cdots, \Delta t_{S}^{\mathrm{crit}}\right)
\end{align}
%
and the critical time step for subdomain $i$ is given by 
%--------------------------------;
%  Equation: Delta t_i critical  ;
%--------------------------------;
\begin{align}
  \Delta t_{i}^{\mathrm{crit}} = \left\{\begin{array}{cl}
      \frac{2}{\omega_{i}^{\mathrm{max}} (1 - 2 \gamma)} & 0 \leq \gamma < 1/2 \\
      +\infty & 1/2 \leq \gamma \leq 1
    \end{array}\right.
\end{align}
%
where $\omega_{i}^{\mathrm{max}}$ is the maximum eigenvalue of the generalized eigenvalue problem 
%--------------------------------;
%  Equation: Eigenvalue problem  ;
%--------------------------------;
\begin{align}
  \label{Eqn:Trapezoidal_GEVP}
  \omega_i \boldsymbol{M}_i \boldsymbol{\phi}_i = \boldsymbol{K}_{i} \boldsymbol{\phi}_i
\end{align}
%
Note that all the eigenvalues $\omega_i$ are real and non-negative \cite{Hughes}.
%
For the chosen time step as described above, the matrices $\boldsymbol{A}_i \; (i = 1, \cdots, S)$ 
(defined in equation \eqref{Eqn:Trapezoidal_A_i}) are positive definite. Also, note that the matrices 
$\boldsymbol{A}_i$ are symmetric. 

%=============================================;
%  Subsection: Stability of the d-continuity  ;
%=============================================;
\subsection{Stability of the $\boldsymbol{d}$-continuity method}
\label{Subsec:DD_d_continuity}
Equation \eqref{Eqn:Trapezoidal_d_continuity_DD_domain} implies 
%------------------------------;
%  Equation: Stability Step 1  ;
%------------------------------;
\begin{align}
  \boldsymbol{M}_i \boldsymbol{v}^{(n + \gamma)}_i
  %
  + \boldsymbol{K}_i \boldsymbol{d}^{(n + \gamma)}_i
  % 
  = \boldsymbol{f}_i^{(n + \gamma)} + \boldsymbol{C}_i^{\mathrm{T}} \boldsymbol{\lambda}^{(n + \gamma)} 
\end{align}
%
where $\boldsymbol{\lambda}^{(n + \gamma)} := (1 - \gamma) \boldsymbol{\lambda}^{(n)} 
+ \gamma \boldsymbol{\lambda}^{(n+1)}$; $\boldsymbol{f}_i^{(n + \gamma)} := (1 - \gamma) 
\boldsymbol{f}_i^{(n)} + \gamma \boldsymbol{f}_i^{(n+1)}$; and similar expressions for 
$\boldsymbol{d}_i^{(n+\gamma)}$ and $\boldsymbol{v}_i^{(n + \gamma)}$.
%
Using equations \eqref{Eqn:Trapezoidal_d_continuity_DD_trapezoidal}, \eqref{Eqn:Trapezoidal_x_gamma} 
and \eqref{Eqn:Trapezoidal_A_i}; the above equation can be written as 
%------------------------------;
%  Equation: Stability Step 2  ;
%------------------------------;
\begin{align}
  \frac{1}{\Delta t} \boldsymbol{A}_i \left[\boldsymbol{d}^{(n)}_i \right] 
  % 
  + \boldsymbol{K}_i \left\{\boldsymbol{d}^{(n)}_i\right\}
  % 
  = \boldsymbol{f}_i^{(n + \gamma)} + \boldsymbol{C}_i^{\mathrm{T}} \boldsymbol{\lambda}^{(n + \gamma)}
\end{align}
%
Premultiplying the above equation by the vector $\left\{\boldsymbol{d}_i^{(n)}\right\}$,  
using the identity given in equation \eqref{Eqn:Trapezoidal_Symmetric_S}, and then summing 
over all $S$ subdomains; we get 
%------------------------------;
%  Equation: Stability Step 3  ;
%------------------------------;
\begin{align}
  \sum_{i = 1}^{S} \frac{1}{2 \Delta t} \left[{\boldsymbol{d}^{(n)}_i}^{\mathrm{T}}
    \boldsymbol{A}_i \boldsymbol{d}^{(n)}_i \right] 
  %
  + \sum_{i=1}^{S} {\left\{\boldsymbol{d}_{i}^{(n)}\right\}}^\mathrm{T} 
  \boldsymbol{K}_i \left\{\boldsymbol{d}^{(n)}_i\right\}
  % 
  = \sum_{i=1}^{S} {\left\{\boldsymbol{d}_i^{(n)}\right\}}^{\mathrm{T}} 
  \left(\boldsymbol{f}_i^{(n + \gamma)} + \boldsymbol{C}_i^{\mathrm{T}} \boldsymbol{\lambda}^{(n + \gamma)}\right) 
\end{align}
%
For stability analysis, one assumes the externally applied forces to be zero (i.e., 
$\boldsymbol{f}_i^{(n)} = \boldsymbol{0}; \; \forall i = 1,\cdots,S; \; \forall n$) 
\cite{Hughes}. Thus, we have
%------------------------------;
%  Equation: Stability Step 2  ;
%------------------------------;
\begin{align}
  \sum_{i = 1}^{S} \frac{1}{2 \Delta t} \left[{\boldsymbol{d}^{(n)}_i}^{\mathrm{T}}
    \boldsymbol{A}_i \boldsymbol{d}^{(n)}_i \right] 
  %
  + \sum_{i=1}^{S} {\left\{\boldsymbol{d}_{i}^{(n)}\right\}}^\mathrm{T} 
  \boldsymbol{K}_i \left\{\boldsymbol{d}^{(n)}_i\right\}
  % 
  = \sum_{i=1}^{S} {\left\{\boldsymbol{d}_i^{(n)}\right\}}^{\mathrm{T}} 
  \boldsymbol{C}_i^{\mathrm{T}} \boldsymbol{\lambda}^{(n + \gamma)}
\end{align}
%
By invoking the fact that the matrices $\boldsymbol{K}_i \; (i = 1, \cdots , S)$ 
are positive semidefinite, we conclude that 
%------------------------------;
%  Equation: Stability Step 3  ;
%------------------------------;
\begin{align}
  \sum_{i = 1}^{S} \frac{1}{2 \Delta t} \left[{\boldsymbol{d}^{(n)}_i}^{\mathrm{T}}
    \boldsymbol{A}_i \boldsymbol{d}^{(n)}_i \right] 
  % 
  \leq \sum_{i = 1}^{S} {\left\{\boldsymbol{d}^{(n)}_i \right\}}^{\mathrm{T}} \boldsymbol{C}_i^{\mathrm{T}} 
  \boldsymbol{\lambda}^{(n + \gamma)} 
  %
  = {\boldsymbol{\lambda}^{(n + \gamma)}}^{\mathrm{T}} \sum_{i=1}^{S} \boldsymbol{C}_i \left\{\boldsymbol{d}^{(n)}_i\right\} 
\end{align}
%
Using the linearity of the average operator (which allows us to interchange the 
summation and average operation), and the $\boldsymbol{d}$-continuity given by 
equation \eqref{Eqn:Trapezoidal_d_continuity_DD_kinematic}; we conclude that 
%------------------------------;
%  Equation: Stability Step 4  ;
%------------------------------;
\begin{align}
 \sum_{i = 1}^{S} \frac{1}{2 \Delta t} \left[{\boldsymbol{d}^{(n)}_i}^{\mathrm{T}}
   \boldsymbol{A}_i \boldsymbol{d}^{(n)}_i \right] \leq 0 \quad \forall n
\end{align}
%
Using the definition and linearity of the jump operator, we conclude 
\begin{align}
  \sum_{i=1}^{S}{\boldsymbol{d}_i^{(n+1)}}^{\mathrm{T}}\boldsymbol{A}_{i} \boldsymbol{d}_i^{(n+1)} \leq 
  \sum_{i=1}^{S} {\boldsymbol{d}_i^{(n)}}^{\mathrm{T}}\boldsymbol{A}_{i} \boldsymbol{d}_i^{(n)} 
  \leq \cdots \leq 
  \sum_{i=1}^{S} {\boldsymbol{d}_i^{(0)}}^{\mathrm{T}}\boldsymbol{A}_{i} \boldsymbol{d}_i^{(0)} 
\end{align}
%
Since $\forall i = 1, \cdots, S$ the initial vectors $\boldsymbol{d}_i^{(0)}$ are bounded 
and the matrices $\boldsymbol{A}_i$ are positive definite; we conclude that the vectors 
$\boldsymbol{d}_i^{(n)} \; (i = 1, \cdots, S)$ are bounded $\forall n$. This implies that, 
from the trapezoidal equation  \eqref{Eqn:Trapezoidal_d_continuity_DD_trapezoidal}, the 
vectors $\boldsymbol{v}_i^{(n+\gamma)} := (1 - \gamma) \boldsymbol{v}_i^{(n)} + \gamma 
\boldsymbol{v}_i^{(n+1)} \; (i = 1, \cdots, S)$ are also bounded $\forall n$. Under zero 
external force the subdomain governing equation \eqref{Eqn:Trapezoidal_d_continuity_DD_domain} 
implies 
%------------------------------;
%  Equation: Stability Step 5  ;  
%------------------------------;
\begin{align}
  \label{Eqn:DD_d_continuity_step5}
  \boldsymbol{M}_i \boldsymbol{v}_i^{(n + \gamma)} + \boldsymbol{K}_i \boldsymbol{d}_i^{(n + \gamma)} 
  = \boldsymbol{C}_i^{\mathrm{T}} \boldsymbol{\lambda}^{(n + \gamma)}, \quad \forall i
\end{align}
%
Since $\boldsymbol{d}_i^{(n)}$ (and hence $\boldsymbol{d}_i^{(n + \gamma)}$) and 
$\boldsymbol{v}_i^{(n + \gamma)}$ are bounded, from equation \eqref{Eqn:DD_d_continuity_step5} 
we conclude that the Lagrange multipliers $\boldsymbol{\lambda}^{(n+\gamma)}$ are also bounded 
$\forall n$. 

But the proof of stability is not yet complete as we have not said anything about the 
boundedness of $\boldsymbol{v}_i^{(n)}$ and $\boldsymbol{\lambda}_i^{(n)}$ and these 
quantities are used to advance the solution. Before we comment on the boundedness of 
rates and Lagrange multipliers at integer time levels $t_n$, we state and prove the 
following general result, which will be useful in assessing stability of coupling 
algorithms. We employ the standard notation used in mathematical analysis. To avoid 
ambiguity, let $\mathbb{N} := \left\{0,1,2, \cdots\right\}$.
%----------------------------------------;
%  Proposition: Proposition on sn_gamma  ;
%----------------------------------------;
\begin{proposition}
  \label{Proposition:DD_Proposition_on_sn_gamma}
  Let $\left(s^{(n)}\right)_{n \in \mathbb{N}}$ be a sequence of real numbers and let 
  $s^{(n + \gamma)} := (1 - \gamma) s^{(n)} + \gamma s^{(n+1)}$, where $0 \leq \gamma 
  \leq 1$. If the element $s^{(0)}$ and the sequence $\left(s^{(n + \gamma)}
  \right)_{n \in \mathbb{N}}$ are bounded, then for any $\gamma > 1/2$ the (original) 
  sequence $\left(s^{(n)}\right)_{n \in \mathbb{N}}$ is also bounded. 
\end{proposition}
%--------------------------------------------;
%  Proof: Proof of proposition on s_n_gamma  ;
%--------------------------------------------;
\begin{proof}
We split the proof into two different cases: $\gamma = 1$ and $1/2 < \gamma < 1$.

\textit{First case $(\gamma = 1)$}: The proof is trivial as in this case $s^{(n + \gamma)} 
= s^{(n+1)}$. The sequence $\left(s^{(n)}\right)_{n \in \mathbb{N}}$ can be obtained by 
augmenting the element $s^{(0)}$ at the start of the sequence 
$\left(s^{(n + \gamma)}\right)_{n \in \mathbb{N}}$. Since the element $s^{(0)}$ and the 
sequence $\left(s^{(n + \gamma)}\right)_{n \in \mathbb{N}}$ are bounded, we conclude that 
the original sequence $\left(s^{(n)}\right)_{n \in \mathbb{N}}$ is also bounded. 

\textit{Second case $(1/2 < \gamma < 1)$}: Construct a new sequence $\left(c^{(n)}\right)_{n \in \mathbb{N}}$ 
such that $c^{(n)} = \left|s^{(n)}\right|$. If $\left(s^{(n)}\right)_{n \in \mathbb{N}}$ is bounded then 
$\left(c^{(n)}\right)_{n \in \mathbb{N}}$ is also bounded and vice-versa. We now prove the proposition 
by the method of contradiction. 

Assume that the sequence $\left(c^{(n)}\right)_{n \in \mathbb{N}}$ is unbounded. Then we can 
find a strictly increasing unbounded subsequence $\left(c^{(n_k)}\right)_{k \in \mathbb{N}} 
\; (n_k \in \mathbb{N}, 0 \leq n_1 < n_2 < \cdots)$ such that 
\begin{align}
  & 0 < c^{(n_1)} < c^{(n_2)} < \cdots \rightarrow \infty \quad \mathrm{and} \\
  \label{Eqn:Trapezoidal_cm_leq_cnk}
  & c^{(m)} < c^{(n_k)} \quad  \forall m < n_k, m \in \mathbb{N}
\end{align}
%
Since the sequence $\left(s^{(n + \gamma)}\right)_{n \in \mathbb{N}}$ is bounded, we can find 
$0 < M \in \mathbb{R}$ such that 
\begin{align}
  \label{Eqn:Trapezoidal_sngamma_leq_M}
  \left|s^{(n + \gamma)}\right| < M \quad \forall n
\end{align}
Since the subsequence $\left(c^{(n_k)}\right)_{k \in \mathbb{N}}$ is strictly increasing and 
unbounded, we can find an element of this subsequence such that 
\begin{align}
  \label{Eqn:Trapezoidal_cnp1_geq_M}
  c^{(n_p)} \geq \frac{1}{2 \gamma - 1} M, \quad p \in \mathbb{N}
\end{align}
%
Since $1/2 < \gamma < 1$ (and, therefore $\gamma > 2 \gamma - 1$), from equations 
\eqref{Eqn:Trapezoidal_sngamma_leq_M} and \eqref{Eqn:Trapezoidal_cnp1_geq_M} we have  
\begin{align}
  \label{Eqn:Trapezoidal_main_inequality}
  \gamma c^{(n_p)} > (2 \gamma - 1) c^{(n_p)} \geq M >  \left|s^{(n + \gamma)}\right| \geq 0 \quad \forall n
\end{align}
%

Using the definition of $s^{(n_p - 1 + \gamma)}$ we have 
\begin{align}
  c^{(n_p - 1)} = \left|s^{(n_p - 1)}\right| &= \frac{1}{1 - \gamma} \left|s^{(n_p - 1 + \gamma)} - \gamma s^{(n_p)}\right| 
\end{align}
%
By using the triangle inequality (and noting that $c^{(n_p)} := |s^{(n_p)}|$) we conclude that 
\begin{align}
  c^{(n_p - 1)} \geq \frac{1}{1 - \gamma} \left|\gamma \left|s^{(n_p)}\right| - \left|s^{(n_p - 1 + \gamma)}\right| \right| 
  = \frac{1}{1 - \gamma} \left|\gamma c^{(n_p)} - \left|s^{(n_p - 1 + \gamma)}\right| \right| 
\end{align}
%
By using equation \eqref{Eqn:Trapezoidal_main_inequality} we obtain 
\begin{align} 
  c^{(n_p - 1)} > \frac{1}{1 - \gamma} \left|\gamma c^{(n_p)} - (2 \gamma - 1) c^{(n_p)}\right| = c^{(n_p)} 
\end{align}
%
which is a contradiction as it violates equation \eqref{Eqn:Trapezoidal_cm_leq_cnk}. This 
implies that the sequence $\left(c^{(n)}\right)_{n \in \mathbb{N}}$ is bounded, and so should 
be the sequence $\left(s^{(n)}\right)_{n \in \mathbb{N}}$. This completes the proof. 
\end{proof}
%-----------------------------------------;
%  Remark: Remark on 0 leq gamma leq 1/2  ; 
%-----------------------------------------;
\begin{remark}
  \label{Remark:DD_Remark_on_gamma_leq_dot5}
  The result proved in Proposition \ref{Proposition:DD_Proposition_on_sn_gamma}, in general, 
  cannot be extended to $0 < \gamma \leq 1/2$. Counterexamples for the cases $0 < \gamma 
  < 1/2$ and $\gamma = 1/2$ are given in figures \ref{Fig:DD_Unstable_sequence_gamma_leq_dot5} 
  and \ref{Fig:DD_Unstable_sequence_gamma_dot5}, respectively. As discussed in Remark 
  \ref{Remark:Trapezoidal_forward_Euler_ill_posed}, the forward Euler $(\gamma = 0)$ is 
  not well-posed under the $\boldsymbol{d}$-continuity method. 
  % 
  This implies that, under the $\boldsymbol{d}$-continuity domain decomposition method, many of 
  the popular time stepping schemes from the generalized trapezoidal family (e.g., the forward 
  Euler and midpoint rule) are unstable. The midpoint rule $(\gamma = 1/2)$ is unconditionally 
  stable for linear first-order ODEs. But for linear index-2 DAEs, the midpoint rule can be 
  unstable (and is right on the boundary of the instability region). 
\end{remark}

%---------------------------------------------;
%  Figure: Unstable sequence for gamma < 1/2  ;
%---------------------------------------------;
\begin{figure}
  \psfrag{0}{$0$}
  \psfrag{1}{$1$}
  \psfrag{2}{$2$}
  \psfrag{3}{$3$}
  \psfrag{4}{$4$}
  \psfrag{n}{$n$}
  \psfrag{g}{$\gamma$}
  \psfrag{gl}{$\gamma < 1/2$}
  \psfrag{s0}{$s^{(0)}$}
  \psfrag{s1}{$s^{(1)}$}
  \psfrag{s2}{$s^{(2)}$}
  \psfrag{s3}{$s^{(3)}$}
  \psfrag{sn}{$s^{(n)}$}
  \psfrag{sngamma}{$s^{(n + \gamma)}, \forall n$}
  \includegraphics[scale=0.7]{Figures/Unstable_Sequence.eps}
  \caption{A counterexample for the case $0 \leq \gamma < 1/2$. The figure presents an example 
    in which the (constant) sequence $(s^{(n + \gamma)})_{n \in \mathbb{N}}$ is bounded but 
    $(s^{(n)})_{n \in \mathbb{N}}$ is unbounded. The elements of $(s^{(n+ \gamma)})_{n \in 
      \mathbb{N}}$ are indicated using filled squares, and those of $(s^{(n)})_{n \in 
      \mathbb{N}}$ are indicated using circles. 
    Recall that $s^{(n + \gamma)} := (1 - \gamma) s^{(n)} + \gamma s^{(n+1)}, \; \forall n$. 
  \label{Fig:DD_Unstable_sequence_gamma_leq_dot5}} 
\end{figure}

%---------------------------------------------;
%  Figure: Unstable sequence for gamma = 1/2  ;
%---------------------------------------------;
\begin{figure}
  \begin{align*}
    \begin{array}{c|cccccc} 
      n & 0 & 1 & 2 & 3 & 4 & \cdots \\ \hline
      s^{(n + 1/2)} & +1 & -1 & +1 & -1 & +1 & \cdots \\
      s^{(n)} & 0 & +2 & -4 & +6 & -8 & \cdots  
    \end{array}
  \end{align*}
  \caption{A counterexample for $\gamma = 1/2$. The sequence $\left(s^{(n + 1/2)}\right)_{n \in \mathbb{N}}, 
    \; s^{(n + 1/2)} := \left(s^{(n)} + s^{(n+1)}\right)/2,$ is bounded but the sequence 
    $\left(s^{(n)}\right)_{n \in \mathbb{N}}$ is unbounded. \label{Fig:DD_Unstable_sequence_gamma_dot5}}
\end{figure}

Returning to the proof of stability of the $\boldsymbol{d}$-continuity domain decomposition method, 
we have proved that $\boldsymbol{v}_i^{(n + \gamma)}$ and $\boldsymbol{\lambda}^{(n + \gamma)}$ are 
bounded $\forall i$ and $\forall n$. Applying Proposition \ref{Proposition:DD_Proposition_on_sn_gamma} 
for individual components of the vectors $\boldsymbol{v}_{i}^{(n + \gamma)}$ and 
$\boldsymbol{\lambda}^{(n + \gamma)}$, we can conclude that for $1/2 < \gamma \leq 1$ the vectors 
$\boldsymbol{v}_i^{(n)}$ and $\boldsymbol{\lambda}^{(n)}$ are bounded $\forall i$ and $\forall n$. 
As shown mathematically in Remark \ref{Remark:DD_Remark_on_gamma_leq_dot5}, the quantities 
$\boldsymbol{v}_i^{(n)}$ and $\boldsymbol{\lambda}^{(n)}$ may not be bounded when $0 \leq \gamma 
\leq 1/2$. In a later subsection we will present physical systems that, in fact, exhibit this kind 
of (numerical) unbounded behavior for $\gamma \leq 1/2$ under the $\boldsymbol{d}$-continuity method. 
This completes the stability analysis of the $\boldsymbol{d}$-continuity method. 

%==================================================;
%  Subsection: Stability of modified d-continuity  ;
%==================================================;
\subsection{Stability of modified $\boldsymbol{d}$-continuity method}
\label{Subsec:DD_stability_modified_d_continuity}
The majority of the proof for this method is identical to the initial part of the proof for 
the $\boldsymbol{d}$-continuity method (presented in subsection \ref{Subsec:DD_d_continuity}) 
up to the step where we deduced that the vectors $\boldsymbol{\lambda}^{(n+ \gamma)}$ and 
$\boldsymbol{v}_i^{(n+\gamma)}$ are bounded. The only additional thing we have to prove is 
the boundedness of the vectors $\boldsymbol{\lambda}^{(n)}$ and $\boldsymbol{v}_i^{(n)}$, 
which is a direct consequence of the triangle inequality. To wit, using equation 
\eqref{Eqn:DD_modified_lambda_interpolation} (and also see Figure 
\ref{Fig:DD_interpolation_lambda}) we have 
%---------------------------------;
%  Equation: Triangle inequality  ;
%---------------------------------;
\begin{align}
  \label{Eqn:DD_triangle_inequality}
  \left\|\boldsymbol{\lambda}^{(n)}\right\| = 
  \left\|\gamma \boldsymbol{\lambda}^{(n-1+\gamma)} + 
    (1 - \gamma) \boldsymbol{\lambda}^{(n + \gamma)}\right\| 
  %
  \leq \gamma \left\|\boldsymbol{\lambda}^{(n-1+\gamma)}\right\| + 
  (1 - \gamma) \left\|\boldsymbol{\lambda}^{(n+\gamma)}\right\| 
\end{align}
%
Since the vectors $\boldsymbol{\lambda}^{(n+\gamma)}$ are bounded $\forall n$, from the above equation 
it is evident that the Lagrange multipliers at integral time levels $\boldsymbol{\lambda}^{(n)}$ are 
bounded $\forall n$. Using a similar reasoning, since the vectors $\boldsymbol{v}_i^{(n+\gamma)}$ are 
bounded $\forall n$, the rates at the integer time levels $\boldsymbol{v}_i^{(n)}$ are also bounded. 
(Note that the vectors $\boldsymbol{d}_i^{(n)}$ are also bounded, which has been proven in subsection 
\ref{Subsec:DD_d_continuity}.) This means that under this method all quantities of interest are 
bounded. This completes the stability analysis of the modified $\boldsymbol{d}$-continuity method. 

Note that, as discussed in Remark \ref{Remark:Trapezoidal_forward_Euler_ill_posed}, the forward 
Euler $(\gamma = 0)$ is not well-posed under the modified $\boldsymbol{d}$-continuity method. All 
other time integrators from the generalized trapezoidal family $(0 < \gamma \leq 1)$ can be employed 
and are stable under the modified $\boldsymbol{d}$-continuity domain decomposition method. 

%------------------------------------------------------------------------;
%  Remark: Comments on the backward Euler with d-continuity constraints  ;
%------------------------------------------------------------------------;
\begin{remark} 
  \label{Remark:DD_backward_Euler_d_continuity}
  For the $\boldsymbol{d}$-continuity and modified $\boldsymbol{d}$-continuity domain 
  decomposition methods, with backward Euler $(\gamma = 1)$ one can achieve the continuity 
  of both temperatures and temperature rates along the subdomain interface. To wit, the 
  $\boldsymbol{d}$-continuity constraints (which are basically the continuity of temperatures 
  along the interface, and are given by equation \eqref{Eqn:Trapezoidal_d_continuity_DD_kinematic} 
  or \eqref{Eqn:Trapezoidal_modified_d_continuity_DD_kinematic}) imply 
  %-----------------------------------;
  %  Equation: backward Euler Step 1  ;
  %-----------------------------------;
  \begin{align}
    \sum_{i = 1}^{S} \boldsymbol{C}_i \left[\boldsymbol{d}_i^{(n-1)}\right] = \boldsymbol{0}, \; \forall n
  \end{align}
  % 
  For backward Euler we have $\left[\boldsymbol{d}_i^{(n-1)}\right] = \Delta t \boldsymbol{v}_i^{(n)}$. 
  This implies the continuity of rates along the subdomain interface.
  %-----------------------------------;
  %  Equation: backward Euler Step 2  ;
  %-----------------------------------;
  \begin{align}
    \sum_{i = 1}^{S} \boldsymbol{C}_i \boldsymbol{v}_i^{(n)} = \boldsymbol{0}, \; \forall n
  \end{align}
  % 
\end{remark}

%=============================================;
%  Subsection: Stability of the v-continuity  ;
%=============================================;
\subsection{Stability of the $\boldsymbol{v}$-continuity method}
We follow a similar procedure employed in subsection \ref{Subsec:DD_d_continuity}. Using equations 
\eqref{Eqn:Trapezoidal_d_continuity_DD_domain}-\eqref{Eqn:Trapezoidal_d_continuity_DD_trapezoidal} 
(and as usual neglecting the external forcing function for stability analysis \cite{Hughes}; i.e., 
$\boldsymbol{f}_i^{(n)} = \boldsymbol{0}$) one obtains 
%------------------------------;
%  Equation: Stability Step 1  ;
%------------------------------;
\begin{align}
  \sum_{i = 1}^{S} \frac{1}{2} \left[{\boldsymbol{v}^{(n)}_i}^{\mathrm{T}}
    \boldsymbol{A}_i \boldsymbol{v}^{(n)}_i \right] 
  %
  + \sum_{i=1}^{S} \Delta t {\left\{\boldsymbol{v}_{i}^{(n)}\right\}}^\mathrm{T} 
  \boldsymbol{K}_i \left\{\boldsymbol{v}^{(n)}_i\right\}
  % 
  = \sum_{i=1}^{S} {\left\{\boldsymbol{v}_i^{(n)}\right\}}^{\mathrm{T}} 
  \boldsymbol{C}_i^{\mathrm{T}} \left[\boldsymbol{\lambda}^{(n)}\right]
\end{align}
%
Since  the matrices $\boldsymbol{K}_i \; (i = 1, \cdots , S)$ are positive 
semidefinite, and $\Delta t > 0$; we conclude 
%------------------------------;
%  Equation: Stability Step 2  ;
%------------------------------;
\begin{align}
  \sum_{i = 1}^{S} \frac{1}{2} \left[{\boldsymbol{v}^{(n)}_i}^{\mathrm{T}}
    \boldsymbol{A}_i \boldsymbol{v}^{(n)}_i \right] 
  % 
  \leq \sum_{i = 1}^{S} {\left\{\boldsymbol{v}^{(n)}_i \right\}}^{\mathrm{T}} \boldsymbol{C}_i^{\mathrm{T}} 
  \left[\boldsymbol{\lambda}^{(n)} \right] 
  %
  = {\left[\boldsymbol{\lambda}^{(n)}\right]}^{\mathrm{T}} \sum_{i=1}^{S} 
  \boldsymbol{C}_i \left\{\boldsymbol{v}^{(n)}_i\right\} 
\end{align}
%
Using the $\boldsymbol{v}$-continuity given by equation 
\eqref{Eqn:Trapezoidal_v_continuity_DD_kinematic} we conclude that 
%------------------------------;
%  Equation: Stability Step 3  ;
%------------------------------;
\begin{align}
 \sum_{i = 1}^{S} \frac{1}{2} \left[{\boldsymbol{v}^{(n)}_i}^{\mathrm{T}}
   \boldsymbol{A}_i \boldsymbol{v}^{(n)}_i \right] \leq 0 \quad \forall n
\end{align}
%
Using the definition and linearity of the jump operator, we conclude 
\begin{align}
  \sum_{i=1}^{S}{\boldsymbol{v}_i^{(n+1)}}^{\mathrm{T}}\boldsymbol{A}_{i} \boldsymbol{v}_i^{(n+1)} \leq 
  \sum_{i=1}^{S} {\boldsymbol{v}_i^{(n)}}^{\mathrm{T}}\boldsymbol{A}_{i} \boldsymbol{v}_i^{(n)} 
  \leq \cdots \leq 
  \sum_{i=1}^{S} {\boldsymbol{v}_i^{(0)}}^{\mathrm{T}}\boldsymbol{A}_{i} \boldsymbol{v}_i^{(0)} 
\end{align}
%
Since $\forall i = 1, \cdots, S$ the initial vectors $\boldsymbol{v}_i^{(0)}$ are bounded and 
the matrices $\boldsymbol{A}_i$ are positive definite; we conclude that $\boldsymbol{v}_i^{(n)}$ 
are bounded $\forall n$. This implies that, from the trapezoidal equation 
\eqref{Eqn:Trapezoidal_v_continuity_DD_trapezoidal}, $\left[\boldsymbol{d}_i^{(n)}\right]$ is 
bounded. Then, from the subdomain governing equation \eqref{Eqn:Trapezoidal_v_continuity_DD_domain}, 
we conclude that $\left[\boldsymbol{\lambda}_i^{(n)}\right]$ is also bounded. 

For the $\boldsymbol{v}$-continuity domain decomposition method, solely based on the energy 
method, one cannot infer the boundedness of the quantities $\boldsymbol{d}_i^{(n)}$ and 
$\boldsymbol{\lambda}^{(n)}$. Also, there can be drift in the continuity of temperatures 
along the subdomain interface. That is, $\sum_{i = 1}^{S} \boldsymbol{C}_i \boldsymbol{d}_i^{(n)} 
\neq \boldsymbol{0}$. This drift may grow over time due to round-off errors. As discussed 
earlier, one of the ways to control the drift is to employ the Baumgarte stabilization. In 
next subsection, we discuss the stability of the Baumgarte constraint stabilization in the 
context of index-2 linear first-order transient systems.  
%------------------------------------------------------;
%  Remark: Remark on forward Euler under v-continuity  ;
%------------------------------------------------------;
\begin{remark}
  Note that, unlike the $\boldsymbol{d}$-continuity and modified $\boldsymbol{d}$-continuity 
  methods, one can employ the forward Euler method $(\gamma = 0)$ in individual subdomains 
  under the $\boldsymbol{v}$-continuity domain decomposition method. 
\end{remark}

%=============================================================================;
%  Subsection: Stability of Baumgarte stabilized domain decomposition method  ;
%=============================================================================;
\subsection{Stability of Baumgarte stabilized domain decomposition method}
\label{Subsec:Trapezoidal_Baumgarte_theory}
We start the stability analysis by rewriting the kinematic constraints. To this end, 
equation \eqref{Eqn:Trapezoidal_Baumgarte_kinematic} implies that 
%---------------------------------------------;
%  Equation: Baumgarte constraints jump form  ;
%---------------------------------------------;
\begin{align}
  \sum_{i=1}^{S} \boldsymbol{C}_i \left(\left[\boldsymbol{v}_i^{(n)}\right] + 
    \frac{\alpha}{\Delta t} \left[\boldsymbol{d}_i^{(n)}\right] \right) = \boldsymbol{0}
\end{align}
%
By using the kinematic constraints given by equation \eqref{Eqn:Trapezoidal_Baumgarte_kinematic} 
and identity \eqref{Eqn:Trapezoidal_x_gamma} we get 
%-----------------------------------------;
%  Equation: Final Baumgarte constraints  ;
%-----------------------------------------;
\begin{align}
  \label{Eqn:Trapezoidal_final_Baumgarte_constraints}
  \sum_{i=1}^{S} \boldsymbol{C}_i \left(\alpha^{*} \left[\boldsymbol{v}_i^{(n)}\right] + 
    \alpha \left\{\boldsymbol{v}_i^{(n)}\right\}\right) = \boldsymbol{0}
\end{align}
%
where the (dimensionless) parameter $\alpha^{*}$ is introduced for convenience, 
and is defined as 
%--------------------------------------;
%  Equation: Definition of alpha_star  ;
%--------------------------------------;
\begin{align}
  \label{Eqn:Trapezoidal_alpha_star}
  \alpha^{*} := 1 + \alpha \left(\gamma - \frac{1}{2}\right)
\end{align}

We now rewrite the subdomain equation in a manner similar to what we did above for the 
kinematic constraints. Equation \eqref{Eqn:Trapezoidal_Baumgarte_domain} implies that
%-----------------------------------;
%  Equation: Equilibrium jump form  ;
%-----------------------------------;
\begin{align}
  \label{Eqn:Trapezoidal_equilibrium_jump_form}
  \boldsymbol{M}_i \left[\boldsymbol{v}_i^{(n)}\right] + \boldsymbol{K}_i \left[\boldsymbol{d}_i^{(n)}\right] = 
  \boldsymbol{C}_i^{\mathrm{T}} \left[\boldsymbol{\lambda}^{(n)}\right]
\end{align}
%
By using the trapezoidal equation \eqref{Eqn:Trapezoidal_Baumgarte_trapezoidal} and employing 
the identity \eqref{Eqn:Trapezoidal_x_gamma} we get 
%------------------------------------;
%  Equation: Equilibrium final form  ;
%------------------------------------; 
\begin{align}
  \boldsymbol{M}_i \left[\boldsymbol{v}_i^{(n)}\right] + \Delta t \boldsymbol{K}_i 
  \left( \left(\gamma - \frac{1}{2}\right) \left[\boldsymbol{v}_i^{(n)}\right] + 
    \left\{\boldsymbol{v}_i^{(n)}\right\}\right) = \boldsymbol{C}_i^{\mathrm{T}} 
  \left[\boldsymbol{\lambda}^{(n)}\right] 
\end{align}

Premultiplying both sides of the above equation by $\left(\alpha^{*} \left[\boldsymbol{v}_i^{(n)}
  \right] + \alpha \left\{\boldsymbol{v}_i^{(n)}\right\}\right)$ and then summing over all of the 
subdomains we get 
%------------------------------;
%  Equation: Stability step 1  ;
%------------------------------;
\begin{align}
  &\sum_{i=1}^{S} \left(\alpha^{*} \left[\boldsymbol{v}_i^{(n)}\right] + \alpha 
    \left\{\boldsymbol{v}_i^{(n)}\right\}\right)^{\mathrm{T}} \left(\boldsymbol{M}_i 
  \left[\boldsymbol{v}_i^{(n)}\right] + \Delta t \boldsymbol{K}_i 
  \left(\left(\gamma - 1/2\right) \left[\boldsymbol{v}_i^{(n)}\right] + 
    \left\{\boldsymbol{v}_i^{(n)}\right\}\right)\right)\notag \\
  %
  &= \sum_{i=1}^{S} \left(\alpha^{*} \left[\boldsymbol{v}_i^{(n)}\right] + \alpha 
    \left\{\boldsymbol{v}_i^{(n)}\right\}\right)^{\mathrm{T}} \boldsymbol{C}_i^{\mathrm{T}} 
  \left[\boldsymbol{\lambda}^{(n)}\right] 
  %
  = \left[\boldsymbol{\lambda}^{(n)}\right]^{\mathrm{T}} \sum_{i=1}^{S} \boldsymbol{C}_i 
  \left(\alpha^{*} \left[\boldsymbol{v}_i^{(n)}\right] + \alpha \left\{\boldsymbol{v}_i^{(n)}\right\}\right)    
\end{align}
%
For the Baumgarte stabilized domain decomposition method, using equation 
\eqref{Eqn:Trapezoidal_final_Baumgarte_constraints}, we conclude that 
%------------------------------;
%  Equation: Stability step 2  ;
%------------------------------;
\begin{align}
  \sum_{i=1}^{S} \left(\alpha^{*} \left[\boldsymbol{v}_i^{(n)}\right] + \alpha 
    \left\{\boldsymbol{v}_i^{(n)}\right\}\right)^{\mathrm{T}} \left(\boldsymbol{M}_i 
  \left[\boldsymbol{v}_i^{(n)}\right] + \Delta t \boldsymbol{K}_i 
  \left(\left(\gamma - 1/2\right) \left[\boldsymbol{v}_i^{(n)}\right] + 
    \left\{\boldsymbol{v}_i^{(n)}\right\}\right)\right) = 0
\end{align}
%
Using the definition of $\alpha^{*}$ (equation \eqref{Eqn:Trapezoidal_alpha_star}), 
the above equation can be rewritten as 
%------------------------------;
%  Equation: Stability step 3  ;
%------------------------------;
\begin{align}
  \sum_{i=1}^{S} \left(\alpha^{*} \left[\boldsymbol{v}_i^{(n)}\right] + \alpha 
    \left\{\boldsymbol{v}_i^{(n)}\right\}\right)^{\mathrm{T}} \boldsymbol{M}_i 
  \left[\boldsymbol{v}_i^{(n)}\right] 
  % 
  + \Delta t \sum_{i=1}^{S} \left[\boldsymbol{v}_i^{(n)}\right]^{\mathrm{T}} 
  \boldsymbol{K}_i \left(\left(\gamma - 1/2\right) \left[\boldsymbol{v}_i^{(n)}\right] + 
      \left\{\boldsymbol{v}_i^{(n)}\right\}\right) \notag \\
  % 
  + \alpha \Delta t \sum_{i=1}^{S} \left((\gamma - 1/2) \left[\boldsymbol{v}_i^{(n)}\right] + 
    \left\{\boldsymbol{v}_i^{(n)}\right\}\right)^{\mathrm{T}} \boldsymbol{K}_i 
    \left(\left(\gamma - 1/2\right) \left[\boldsymbol{v}_i^{(n)}\right] + 
      \left\{\boldsymbol{v}_i^{(n)}\right\}\right) = 0
\end{align}
%
Since $\alpha > 0$, $\Delta t > 0$ and $\boldsymbol{K}_i$ is positive semidefinite, we conclude 
%------------------------------;
%  Equation: Stability step 4  ;
%------------------------------;
\begin{align}
  \sum_{i=1}^{S} \left(\alpha^{*} \left[\boldsymbol{v}_i^{(n)}\right] + \alpha 
    \left\{\boldsymbol{v}_i^{(n)}\right\}\right)^{\mathrm{T}} \boldsymbol{M}_i 
  \left[\boldsymbol{v}_i^{(n)}\right] 
  % 
  + \Delta t \sum_{i=1}^{S} \left[\boldsymbol{v}_i^{(n)}\right]^{\mathrm{T}} 
  \boldsymbol{K}_i \left(\left(\gamma - 1/2\right) \left[\boldsymbol{v}_i^{(n)}\right] + 
      \left\{\boldsymbol{v}_i^{(n)}\right\}\right) \leq 0
\end{align}
%------------------------------;
%  Equation: Stability step 5  ;
%------------------------------;
By invoking the symmetry of $\boldsymbol{M}_i$, using equation \eqref{Eqn:Trapezoidal_alpha_star}, 
and rearranging the terms we get 
\begin{align}
  \label{Eqn:New_DD_Baum_stab_step5}
  \sum_{i=1}^{S} \left[\boldsymbol{v}_i^{(n)}\right]^{\mathrm{T}} 
  \left(\alpha \boldsymbol{M}_i + \Delta t \boldsymbol{K}_i\right) 
  \left\{\boldsymbol{v}_i^{(n)}\right\} 
  % 
  + \sum_{i=1}^{S} \left[\boldsymbol{v}_i^{(n)}\right]^{\mathrm{T}} 
  \boldsymbol{\tilde{A}}_i \left[\boldsymbol{v}_i^{(n)}\right] \leq 0
\end{align}
%
where the matrix $\boldsymbol{\tilde{A}}_i$ is defined as 
%-------------------------------------;
%  Equation: Definition of A_i_tilde  ;
%-------------------------------------;
\begin{align}
  \label{Eqn:New_DD_definition_of_A_i_tilde}
  \boldsymbol{\tilde{A}}_i := \alpha^{*} \boldsymbol{M}_i + \Delta t 
  \left(\gamma - \frac{1}{2}\right) \boldsymbol{K}_i
\end{align}

If the matrices $\tilde{\boldsymbol{A}}_i \; (i = 1, \cdots, S)$ are positive semidefinite 
(later we will obtain sufficient conditions for the matrix $\tilde{\boldsymbol{A}}_i$ to be 
positive semidefinite) then equation \eqref{Eqn:New_DD_Baum_stab_step5} implies that 
%------------------------------;
%  Equation: Stability step 6  ;
%------------------------------;
\begin{align}
  \sum_{i=1}^S \left[\boldsymbol{v}_i^{(n)}\right]^{\mathrm{T}} 
  \left(\alpha \boldsymbol{M}_i + \Delta t \boldsymbol{K}_i\right) 
  \left\{\boldsymbol{v}_i^{(n)}\right\} \leq 0
\end{align}
%
By invoking identity \eqref{Eqn:Trapezoidal_Symmetric_S} we have 
%------------------------------;
%  Equation: Stability step 7  ;
%------------------------------;
\begin{align}
  &\sum_{i=1}^S \left[\left(\boldsymbol{v}_i^{(n)}\right)^{\mathrm{T}} 
    \left(\alpha \boldsymbol{M}_i + \Delta t \boldsymbol{K}_i\right) 
    \boldsymbol{v}_i^{(n)}\right] \leq 0 \quad \forall n
\end{align}
This implies that 
%------------------------------;
%  Equation: Stability step 8  ;
%------------------------------;
\begin{align}
  \sum_{i=1}^S \left(\boldsymbol{v}_i^{(n+1)}\right)^{\mathrm{T}} \left(\alpha \boldsymbol{M}_i 
    + \Delta t \boldsymbol{K}_i\right) \boldsymbol{v}_i^{(n+1)} \leq \cdots \leq
  \sum_{i=1}^S \left(\boldsymbol{v}_i^{(0)}\right)^{\mathrm{T}} 
  \left(\alpha \boldsymbol{M}_i + \Delta t \boldsymbol{K}_i\right) 
  \boldsymbol{v}_i^{(0)} 
\end{align}
%
Since $\alpha > 0$, $\boldsymbol{M}_i$ is positive definite, and $\boldsymbol{K}_i$ is 
positive semidefinite; the matrix $\alpha \boldsymbol{M}_i + \Delta t \boldsymbol{K}_i$ 
is positive definite. This implies that the vectors $\boldsymbol{v}_i^{(n)}$ are bounded 
$\forall n$ as the (initial) vectors $\boldsymbol{v}_i^{(0)}$ are bounded. This further 
implies that, from the kinematic constraints for the Baumgarte stabilized method (given 
by equation \eqref{Eqn:Trapezoidal_Baumgarte_kinematic}), \emph{the drift in the original 
constraint (i.e., continuity of temperature along the subdomain interface) is also bounded 
(but may not be zero), which is not the case with the $\boldsymbol{v}$-continuity method}. 

To show this (for convenience) let us work with $1$-norm, and the result (boundedness) 
will hold for other norms also (because of equivalence of norms in finite dimensional 
vector spaces). We start with the $1$-norm of the drift in the original constraint, and 
use equation \eqref{Eqn:Trapezoidal_Baumgarte_kinematic} and the triangle inequality:
%-----------------------------------------------------;
%  Equation: Drift is bounded in Baumgarte (Step #1)  ;
%-----------------------------------------------------;
\begin{align}
  \label{Eqn:DD_drift_bounded_step_1} 
  \|\sum_{i=1}^{S} \boldsymbol{C}_i \boldsymbol{d}_i^{(n)}\| 
  = \frac{\Delta t}{\alpha} \|\sum_{i=1}^{S} \boldsymbol{C}_i \boldsymbol{v}_i^{(n)}\| 
  \leq \frac{\Delta t}{\alpha} \sum_{i=1}^{S} \|\boldsymbol{C}_i \boldsymbol{v}_i^{(n)}\| 
\end{align}
%
Now using the definition of matrix-norm, and the boundedness of $\boldsymbol{v}^{(n)}_i$; 
equation \eqref{Eqn:DD_drift_bounded_step_1} can be written as 
%-----------------------------------------------------;
%  Equation: Drift is bounded in Baumgarte (Step #2)  ;
%-----------------------------------------------------;
\begin{align}
  \label{Eqn:DD_drift_bounded_step_2}
  \|\sum_{i=1}^{S} \boldsymbol{C}_i \boldsymbol{d}_i^{(n)}\| 
  \leq \frac{\Delta t}{\alpha} \sum_{i=1}^{S} \| \boldsymbol{C}_i\| \|\boldsymbol{v}_i^{n}\| 
  \leq \frac{\Delta t}{\alpha} \sum_{i=1}^{S} \|\boldsymbol{v}_i^{(n)}\| < C \quad \forall n
\end{align}
%
where $C > 0$ is some constant independent of $n$, and we have used the fact that the 
$1$-norm $\|\boldsymbol{C}_i\|_{1} \leq 1$. (Also recall that if $\boldsymbol{C}_i \neq 
\boldsymbol{0}$, which is the case in this paper, $\|\boldsymbol{C}_i\|_{1} = 1$.) Equation 
\eqref{Eqn:DD_drift_bounded_step_2} implies that \emph{the drift in the original constraint 
is bounded $\forall n$}. 

Similar to the $\boldsymbol{v}$-continuity method, even under the Baumgarte stabilized method, 
one cannot infer anything about the boundedness of $\boldsymbol{d}^{(n)}_i$ or Lagrange multipliers 
$\boldsymbol{\lambda}^{(n)}$ solely based on the energy method. But, for many practical problems 
one often gets bounded numerical results for these quantities. The boundedness of the drift 
in the original constraint is the only additional (but very important) feature that the 
Baumgarte stabilized method has compared to the $\boldsymbol{v}$-continuity method. 

We will now obtain sufficient conditions for the matrix $\tilde{\boldsymbol{A}}_i$ to be 
positive semidefinite (which we have assumed in the stability analysis of this method, see 
the line below equation \eqref{Eqn:New_DD_definition_of_A_i_tilde}). 
%
Using the eigenvectors of the generalized eigenvalue problem \eqref{Eqn:Trapezoidal_GEVP} as 
the basis, the matrix $\tilde{\boldsymbol{A}}_i$ can be diagonalized and obeys the similarity 
%----------------------------;
%  Equation: Similar matrix  ;
%----------------------------;
\begin{align}
  \label{Eqn:Trapezoidal_similar_matrix}
  \tilde{\boldsymbol{A}}_i \sim \alpha^{*} \boldsymbol{I} + \Delta t 
  \left(\gamma - \frac{1}{2}\right) \boldsymbol{\Omega}_i
\end{align}
%
In the above equation, the symbol ``$\sim$'' denotes similarity of matrices, and the matrix 
$\boldsymbol{\Omega}_i$ is defined as
%----------------------------;
%  Equation: Matrix Omega_i  ;
%----------------------------;
\begin{align}
  \boldsymbol{\Omega}_i = \mathrm{diag}\left(\left(\omega_i\right)_1,\cdots, 
    \left(\omega_i\right)_n\right)
\end{align}
%
where $n$ is the size of the (square) matrix $\tilde{\boldsymbol{A}}_i$; and $\left(\omega_i 
\right)_1,\cdots, \left(\omega_i\right)_n$ are the eigenvalues of the generalized eigenvalue 
problem \eqref{Eqn:Trapezoidal_GEVP}. (It is well-known that similar matrices have the same 
characteristic polynomial, and hence the same eigenvalues \cite{Halmos}.)

Since $\boldsymbol{M}_i$ is positive definite and $\boldsymbol{K}_i$ is positive 
semidefinite, the eigenvalues $\left(\omega_i\right)_1,\cdots,\left(\omega_i\right)_n$ 
are all non-negative. This implies that (using equations \eqref{Eqn:Trapezoidal_alpha_star} 
and \eqref{Eqn:Trapezoidal_similar_matrix}, and noting that $\Delta t > 0$) the matrix 
$\tilde{\boldsymbol{A}}_i$ is positive semidefinite unconditionally for $\gamma \geq 1/2$. 
For $\gamma < 1/2$, sufficient conditions for the matrix $\tilde{\boldsymbol{A}}_i$ to be 
positive semidefinite are 
%-------------;
%  Equation:  ;
%-------------;
\begin{align}
  &\alpha^{*} \geq 0 \implies \alpha \leq \frac{1}{|\gamma - 1/2|} \\
  %
  \label{Eqn:Trapezoidal_Baumgarte_t_crit}
  &\Delta t \leq \Delta t_i^{\mathrm{crit}} = \frac{\alpha^{*}}{|\gamma - 1/2| \omega_i^{\mathrm{max}}} = 
  \frac{2}{(1 - 2 \gamma) \omega_i^{\mathrm{max}}} - \frac{\alpha}{\omega_i^{\mathrm{max}}}
\end{align}
%------------------;
%  Remark: Remark  ;
%------------------;
\begin{remark}
  Note that in equation \eqref{Eqn:Trapezoidal_Baumgarte_t_crit} $\Delta t_i^{\mathrm{crit}} 
  \geq 0$ as $\alpha^{*} \geq 0$ and $\omega_i^{\mathrm{max}} \geq 0$. 
\end{remark}

These results imply that the use of Baumgarte stabilization decreases the critical step 
for subdomain $i$ by $\alpha/{\omega_i^{\mathrm{max}}}$ relative to the unconstrained case. 
Summarizing the results, sufficient conditions for the stability of Baumgarte stabilized 
domain decomposition method are  
%-------------------------------------;
%  Equation: Summarizing the results  ;
%-------------------------------------;
\begin{align}
  \label{Eqn:Trapezoidal_Baumgarte_final_result_leq_dot5}
  0 \leq \gamma < 1/2 & \quad \left\{\begin{array}{l}
      \alpha \leq \frac{1}{|\gamma - 1/2|} \\
      \Delta t_i^{\mathrm{crit}} = 
      \frac{2}{(1 - 2 \gamma) \omega_i^{\mathrm{max}}} - 
      \frac{\alpha}{\omega_i^{\mathrm{max}}} 
      % 
    \end{array} \right. \\
  % 
  \label{Eqn:Trapezoidal_Baumgarte_final_result_geq_dot5}
  1/2 \leq \gamma \leq 1 & \quad \left\{\begin{array}{l}
      \alpha < + \infty \\
      \Delta t_i^{\mathrm{crit}} = + \infty
    \end{array} \right. 
\end{align}

%-----------------------------------------;
%  Table: A summary of stability results  ;
%-----------------------------------------;
\begin{table}
  \caption{A summary of stability results \label{Table:DD_stability_results}}
  \begin{tabular}{ll} \hline
    Method & Stability characteristics  \\ \hline
    $\boldsymbol{d}$-continuity & Stable for $1/2 < \gamma \leq 1$. \\ 
    Modified $\boldsymbol{d}$-continuity & Stable for $0 < \gamma \leq 1$. \\ 
    $\boldsymbol{v}$-continuity & Drift on the interface. \\ 
    Baumgarte stabilized & Unconditionally stable for $1/2 \leq \gamma \leq 1$. 
    Stability \\ & conditions for $0 \leq \gamma < 1/2$ are given in Eq. 
    \eqref{Eqn:Trapezoidal_Baumgarte_final_result_leq_dot5}. \\ \hline
  \end{tabular} 
\end{table}

For a quick reference, the stability results derived in this section are 
summarized in Table \ref{Table:DD_stability_results}. In the next section 
we verify the theoretical predictions using numerical experiments. 
